Using Multi-Viewpoint Contracts for Negotiation of Embedded Software Updates

In this paper we address the issue of change after deployment in safety-critical embedded system applications. Our goal is to substitute lab-based verification with in-field formal analysis to determine whether an update may be safely applied. This is challenging because it requires an automated process able to handle multiple viewpoints such as functional correctness, timing, etc. For this purpose, we propose an original methodology for contract-based negotiation of software updates. The use of contracts allows us to cleanly split the verification effort between the lab and the field. In addition, we show how to rely on existing viewpoint-specific methods for update negotiation. We illustrate our approach on a concrete example inspired by the automotive domain.

==> eptcsdata.tex <==
\providecommand{\firstpage}{31}
\providecommand{\publicationstatus}{L. Aceto, A. Francalanza and A. Ingolfsdottir (Eds.):  Workshop on \\ Pre- and Post-Deployment Verification Techniques (PrePost 2016)\\
EPTCS 208, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.208.3}{10.4204/EPTCS.208.3}}
\pdfoutput=1


==> tikz/cpastyles.tex <==
\tikzstyle{task} = [minimum height = 2em, minimum width = 2em, circle, draw, shadow, shadedGray];
\tikzstyle{junction} = [minimum height = 1em, minimum width = 3em, trapezium, draw, shadow, shadedGray, shape border rotate = 270];
\tikzstyle{activates}    = [-angle 60];


==> tikz/topologystyles.tex <==

% declare a new shape for the service interface
\makeatletter
\pgfdeclareshape{openinterface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
}
\pgfdeclareshape{interface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{.95\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
  \foregroundpath{
	 \centerpoint
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
    \pgfutil@tempdimb=\radius%      \pgfutil@tempdima = radius
	 \advance\pgfutil@tempdima by-.25\pgfutil@tempdima%
	 \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+.25\pgfutil@tempdimb}{0pt}}}{\pgfutil@tempdima}
	 \pgfusepath{fill}
  }
}
\makeatother

\tikzstyle{component}    = [minimum height = 2em, minimum width = 2em, rectangle, draw, shadow, shadedGray];
\tikzset{service/.style={draw,
	                      ultra thick,
								 black,
                         interface,
							    minimum width=1em,
							    node distance=1.5cm,
							    rotate=#1},
         service/.default=0
}
\tikzset{openrequirement/.style={draw,
	                          ultra thick,
									  black,
									  openinterface,
									  minimum width=1em,
									  node distance=1.5cm,
    								  rotate=#1},
         openrequirement/.default=0
}
\tikzstyle{openservice}  = [fill, circle, minimum width=.8em, node distance=1.5cm];
\tikzstyle{provides}     = [thick];
\tikzstyle{requires}     = [thick];

\tikzstyle{thread}  = [minimum width=3em, minimum height=1.5em, rounded rectangle, draw, shadow, shadedGray];
\tikzstyle{sync}    = [-triangle 60, thick];
\tikzstyle{async}   = [-angle 60,    thick, dashed];

\tikzstyle{maybe} = [very thick, red, dashed];
\tikzstyle{must} = [very thick, red];

